Threshy: Supporting Safe Usage of Intelligent Web Services

Increased popularity of `intelligent' web services provides end-users with machine-learnt functionality at little effort to developers. However, these services require a decision threshold to be set which is dependent on problem-specific data. Developers lack a systematic approach for evaluating intelligent services and existing evaluation tools are predominantly targeted at data scientists for pre-development evaluation. This paper presents a workflow and supporting tool, Threshy, to help software developers select a decision threshold suited to their problem domain. Unlike existing tools, Threshy is designed to operate in multiple workflows including pre-development, pre-release, and support. Threshy is designed for tuning the confidence scores returned by intelligent web services and does not deal with hyper-parameter optimisation used in ML models. Additionally, it considers the financial impacts of false positives. Threshold configuration files exported by Threshy can be integrated into client applications and monitoring infrastructure. Demo: https://bit.ly/2YKeYhE.

==> figures/tomatoes.tex <==
\begin{figure}[t]
  \centering
  \begin{subfigure}[b]{0.2\linewidth}
    \includegraphics[width=\textwidth]{images/0}
  \end{subfigure}
  \hspace{\fill}
  ~
  \begin{subfigure}[b]{0.2\linewidth}
    \includegraphics[width=\textwidth]{images/1}
  \end{subfigure}
  \hspace{\fill}
  ~
  \begin{subfigure}[b]{0.25\linewidth}
    \includegraphics[width=.5\textwidth]{images/2a}~
    \includegraphics[width=.5\textwidth]{images/2b}
    
    \includegraphics[width=.5\textwidth]{images/2c}~
    \includegraphics[width=.5\textwidth]{images/2d}
  \end{subfigure}
  \caption{Pipeline of Nina's harvesting robot. \textit{Left:}~Photo from harvesting robot's webcam. \textit{Centre:}~Classification detecting different types of tomatoes. \textit{Right:}~Binary classification for ripeness (ripe/unripe) based on (R, G, B values).}% Bottom row is selected as ripe.}%, and sorted into sizes 1--10 using scale classification.}
  \label{fig:tomatoes}
\end{figure}

==> frontmatter.tex <==
\title{Threshy: Supporting safe usage of intelligent web services}


\settopmatter{authorsperrow=4}

\author{Alex Cummaudo}
\email{ca@deakin.edu.au}
\orcid{0000-0001-7878-6283}
\affiliation{%
\department{Applied Artificial Intel. Inst.}
\institution{Deakin University}
\city{Geelong}
\country{Australia}
}

\author{Scott Barnett}
\email{scott.barnett@deakin.edu.au}
\orcid{0000-0002-3187-4937}
\affiliation{%
\department{Applied Artificial Intel. Inst.}
\institution{Deakin University}
\city{Geelong}
\country{Australia}
}

\author{Rajesh Vasa}
\email{rajesh.vasa@deakin.edu.au}
\orcid{0000-0003-4805-1467}
\affiliation{%
\department{Applied Artificial Intel. Inst.}
\institution{Deakin University}
\city{Geelong}
\country{Australia}
}

\author{John Grundy}
\email{john.grundy@monash.edu}
\orcid{0000-0003-4928-7076}
\affiliation{%
\department{Faculty of Inf. Tech.}
\institution{Monash University}
\city{Clayton}
\country{Australia}
}

\begin{abstract}
Increased popularity of `intelligent' web services provides end-users with machine-learnt functionality at little effort to developers. However, these services require a decision threshold to be set which is dependent on problem-specific data. Developers lack a systematic approach for evaluating intelligent services and existing evaluation tools are predominantly targeted at data scientists for pre-development evaluation. This paper presents a workflow and supporting tool, Threshy, to help \textit{software developers} select a decision threshold suited to their problem domain. Unlike existing tools, Threshy is designed to operate in multiple workflows including pre-development, pre-release, and support. Threshy is designed for tuning the confidence scores returned by intelligent web services and does not deal with hyper-parameter optimisation used in ML models. Additionally, it considers the financial impacts of false positives.
Threshold configuration files exported by Threshy can be integrated into client applications and monitoring infrastructure. Demo: \url{\demolink}.
\end{abstract}

\begin{CCSXML}
<ccs2012>
<concept>
<concept_id>10002951.10003260.10003304</concept_id>
<concept_desc>Information systems~Web services</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10010147.10010178</concept_id>
<concept_desc>Computing methodologies~Artificial intelligence</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10011007.10011074.10011075</concept_id>
<concept_desc>Software and its engineering~Designing software</concept_desc>
<concept_significance>500</concept_significance>
</concept>
<concept>
<concept_id>10011007.10011074.10011111</concept_id>
<concept_desc>Software and its engineering~Software post-development issues</concept_desc>
<concept_significance>300</concept_significance>
</concept>
</ccs2012>
\end{CCSXML}

\ccsdesc[500]{Information systems~Web services}
\ccsdesc[500]{Computing methodologies~Artificial intelligence}
\ccsdesc[500]{Software and its engineering~Designing software}
\ccsdesc[300]{Software and its engineering~Software post-development issues}

\keywords{intelligent services, tooling, thresholding, decision theory}

\renewcommand{\shortauthors}{Alex Cummaudo et al.}

\copyrightyear{2020} 
\acmYear{2020} 
\setcopyright{acmlicensed}\acmConference[ESEC/FSE '20]{Proceedings of the 28th ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering}{November 8--13, 2020}{Virtual Event, USA}
\acmBooktitle{Proceedings of the 28th ACM Joint European Software Engineering Conference and Symposium on the Foundations of Software Engineering (ESEC/FSE '20), November 8--13, 2020, Virtual Event, USA}
\acmPrice{15.00}
\acmDOI{10.1145/3368089.3417919}
\acmISBN{978-1-4503-7043-1/20/11}

==> preamble/extended.tex <==
\input{extended/authblk}
\input{extended/bibliography}
\input{extended/extra}
\input{extended/footnotes}
\input{extended/graphics}
\input{extended/listings}
\input{extended/tables}
\input{extended/todo}

==> preamble/extended/authblk.tex <==
% \usepackage{authblk}
% \renewcommand*{\Authsep}{, }
% \renewcommand*{\Authand}{, }
% \renewcommand*{\Authands}{, }
% \renewcommand*{\Affilfont}{\normalsize\normalfont}

==> preamble/extended/bibliography.tex <==
\usepackage{natbib}
\bibliographystyle{ACM-Reference-Format}


==> preamble/extended/footnotes.tex <==
\usepackage[multiple]{footmisc} % Two footnotes at the one point

\newcommand{\footnoteurl}[2]{\footnote{{#1} last accessed #2.}} % URL-cited footnotes

==> preamble/extended/graphics.tex <==
\usepackage{graphicx}
\graphicspath{{images/}{../images/}}


==> preamble/extended/listings.tex <==
\usepackage{listings}
\usepackage{textcomp}
\usepackage{color}
\definecolor{maroon}{rgb}{0.5,0,0}
\definecolor{darkgreen}{rgb}{0,0.5,0}

\renewcommand{\lstlistlistingname}{List of Listings}

\lstset{%
    % Basic design
    basicstyle={\small\ttfamily\color{black}},
    captionpos=t,
    abovecaptionskip=\baselineskip,
    belowcaptionskip=\baselineskip,
    columns=fullflexible,
    showstringspaces=false,
    commentstyle=\color{gray}\upshape,
    frame=l,
    upquote=true,
    % Line numbers
    xleftmargin={0.75cm},
    numbers=left,
    stepnumber=1,
    firstnumber=1,
    numberfirstline=true,
    stringstyle=\color{blue},
    %identifierstyle=\color{maroon},
    commentstyle=\color{darkgreen},
    keywordstyle=\color{red},
    upquote=true,
    breaklines=true,
    postbreak=\mbox{\textcolor{red}{$\hookrightarrow$}\space},
}

\newcommand{\beginlstdelim}[3]
{%
  \def\endlstdelim{#2\egroup}%
  \ttfamily#1\bgroup\color{#3}\aftergroup\endlstdelim%
}

\lstdefinestyle{xml_style}
{
  morestring=[b]",
  moredelim=*[s][\bfseries\color{maroon}]{<}{>},
  moredelim=*[s][\bfseries\color{maroon}]{</}{>},
  morecomment=[s]{<?}{?>},
  morecomment=[s]{<!--}{-->},
}

\lstdefinestyle{json_style}
{
  morestring=[b]",
  comment=[l]{//},
  keywordstyle=\bfseries\color{maroon}
}

\lstdefinelanguage{JSON}
{
  style=json_style
}

\lstdefinelanguage{XML}
{
  style=xml_style
}


==> preamble/extended/tables.tex <==
% Use booktabs
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{makecell}
\newcommand{\tablefit}[1]{\resizebox{\textwidth}{!}{#1}}
\newcommand{\tablefitlandscape}[1]{\resizebox{1.2\paperwidth}{!}{#1}}


==> preamble/extended/todo.tex <==
\usepackage{xcolor}
% \newcommand{\todo}[2][]{{\noindent \color{red} \slshape $\langle$~\textsc{\small\underline{todo}}: \textbf{#2}~{\color{darkgray}\textit{#1}}$\rangle$}}
% \newcommand{\todo}[2][]{\textcolor{blue}{#1}} % Adds introduced text but in blue
\newcommand{\todo}[2][]{#1} % Adds introduced text as normal
% \newcommand{\tonote}[1]{\textbf{\sffamily\footnotesize[#1]}}
\newcommand{\tocite}[1]{\tonote{cite:{#1}}}

==> preamble/simple.tex <==
\usepackage{hyperref}
\input{simple/author}
\input{simple/captions}
\input{simple/cleverref}
\input{simple/geometry}
\input{simple/graphics}
\input{simple/typesetting}

==> preamble/simple/author.tex <==
\author{Alex Cummaudo\\Applied Artificial Intelligence Institute\\Deakin University, Australia}
\date{\today}


==> preamble/simple/captions.tex <==
\usepackage[labelfont=bf]{caption}

==> preamble/simple/cleverref.tex <==
\usepackage[capitalise,noabbrev,nameinlink]{cleveref}
\Crefname{lstlisting}{Listing}{Listings}

==> preamble/simple/geometry.tex <==
\usepackage{geometry}
\newgeometry{top=2.25cm,right=2cm,bottom=2.5cm,left=3cm}


==> preamble/simple/graphics.tex <==
\usepackage{graphicx}
\graphicspath{{images/}{../images/}}


==> preamble/simple/typesetting.tex <==
% Linespread of 1.5 as required by SIT
\linespread{1.5}
% Times new roman package
\usepackage{mathptmx}
% Change font style for sub-sub section
\usepackage{sectsty}
\subsubsectionfont{\normalfont\itshape}
